Fourier matrices for $G(d,1,n)$ from quantum general linear groups

We construct a categorification of the modular data associated with every family of unipotent characters of the spetsial complex reflection group $G(d,1,n)$. The construction of the category follows the decomposition of the Fourier matrix as a Kronecker tensor product of exterior powers of the character table $S$ of the cyclic group of order $d$. The representation of the quantum universal enveloping algebra of the general linear Lie algebra $\mathfrak{gl}_m$, with quantum parameter an even root of unity of order $2d$, provides a categorical interpretation of the matrix $\bigwedge^m S$. We also prove some positivity conjectures of Cuntz at the decategorified level.

==> sections/fourier_ddn.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                    %
% Fourier matrices for G(d,d,n) and categorification %
%                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Fourier matrices for $G(d,d,n)$}
\label{sec:fourier_ddn}

\subsection{Symmetric center of some Deligne tensor products}
\label{sec:cat_fourier_ddn}

As in \cref{sec:cat_fourier_d1n}, we consider of the categories $\mathcal{D}_{\xi^{-1}}$ associated with the representations the quantum enveloping algebra of $\gl_n$ at a root of unity.

We consider the Deligne tensor product $\mathcal{D}_{\underline{n},\xi^{-1}}=\mathcal{D}_{n_1,\xi^{-1}} \boxtimes \ldots \boxtimes \mathcal{D}_{n_r,\xi^{-1}}$ for $\underline{n} = (n_1,\ldots,n_r)$ such that $1\leq n_i \leq d$ and $\sum_{i=1}^nn_i \equiv 0 [d]$. Consider now $\mathcal{E}_{\underline{n},\xi^{-1}}$ the full subcategory with simple objects $X(\underline{\lambda})$ satisfying $\sum_{i=1}^r \langle\lambda_i,\varpi_{n_i}\rangle \equiv 0 [d]$. Thanks to the grading, it is easily seen that the category $\mathcal{E}_{\underline{n},\xi^{-1}}$ is stable under the tensor product and is thus a braided fusion category.

We consider the same categories as those introduced in \cref{sec:cat_fourier_d1n}, but the assumption on the integers $n_1,\ldots,n_r$ will change drastically the structure of the category $\mathcal{E}_{\underline{n},\xi^{-1}}$, notably its symmetric center. As before, since $\varepsilon_i$ is of degree $d$, the objects $\varepsilon_{\underline{\delta}}$ for $\underline{\delta}\in\{0,1\}^d$ are in the symmetric center of $\mathcal{E}_{\underline{n},\xi^{-1}}$. But these objects do not generate the symmetric center of $\mathcal{E}_{\underline{n},\xi^{-1}}$. Let $\varepsilon_{\cycl}$ be the object $X(\varpi_{n_1})\boxtimes \cdots\boxtimes X(\varpi_{n_r})=\det_{n_1,\xi^{-1}}\boxtimes \cdots \boxtimes \det_{n_r,\xi^{-1}}$ which is a simple object of $\mathcal{E}_{\underline{n},\xi^{-1}}$ since $\sum_{i=1}^r n_i \equiv 0 [d]$.

\begin{proposition}
  The symmetric center of $\mathcal{E}_{\underline{n},\xi^{-1}}$ is the full subcategory with simple objects $\varepsilon_{\underline{\delta}}\boxtimes \varepsilon_{\cycl}^{\otimes r}$ for $\underline{\delta}\in\{0,1\}^d$ and $0 \leq r < s$.
\end{proposition}

\begin{proof}
 Once again, we show that a transparent object is invertible, using the same strategy. For a transparent simple object $X(\underline{\lambda})$, we consider and consider for $1 \leq i < j \leq r$ the simple object $Y_{i,j}=X(\underline{\mu}^{(i,j)})$ where
  \[
    \mu_k^{(i,j)} =
    \begin{cases}
      \varpi_1 & \text{ if } k = i,\\
      \varpi_{n_{j}-1}-\varpi_{n_j} & \text{ if } k=j, \\
      0 & \text{ otherwise}.
    \end{cases}
  \]
  The object $Y_{i,j}$ is in $\mathcal{E}_{\underline{n},\xi^{-1}}$. As in the proof of \cref{prop:symmetric_center}, considering decomposition of the tensor product $X(\underline{\lambda})\otimes Y_{i,j}$ shows that both $X(\lambda_i)$ and $X(\lambda_j)$ are invertible and therefore $X(\underline{\lambda})$ is also invertible.
  
  We hence may and will suppose that for every $1 \leq i \leq r$, there exists $1 \leq l_i \leq n_i$ and $s_i \in \mathbb{Z}$ such that $\lambda_i = (d-n_i)\varpi_{l_i} + s_i \varpi_{n_i}$. Then, as in the proof of \cref{prop:symmetric_center}, $X(\underline{\lambda})$ is transparent if and only if for all $\underline{\lambda}$ such that $\sum_{i=1}^r \langle\lambda_i,\varpi_{n_i}\rangle \equiv 0 [d]$, we have
 \[
   \sum_{k=1}^r (s_k-l_k)\langle\lambda_k,\varpi_{n_k}\rangle \equiv 0 [d].
 \]
 Choosing $\underline{\lambda} = \underline{\mu}^{(i,j)}$ as above, we find that $s_i-l_i \equiv s_j-l_j [d]$. Therefore, the value residue class modulo $d$ of $s_i-l_i$ does not depend on $i$. Let $0 \leq t < d$ and $m_i\in\mathbb{Z}$ be such that $s_i-l_i = m_i d + t$. Then we have
 \[
   X((d-n_i)\varpi_{l_i} + s_i \varpi_{n_i}) \simeq \det_{n_i,\xi^{-1}}^{\otimes d m_i +t}\otimes \varepsilon_{n_i}^{\otimes l_i},
 \]
 and therefore, since $\det_{n_i,\xi^{-1}}^{\otimes d}\simeq \varepsilon_{n_i}^{\otimes n_i}$, we obtain that $X(\underline{\lambda})$ is isomorphic in $\mathcal{E}_{\underline{n},\xi^{-1}}$ to the tensor product of $\varepsilon_{\cycl}^{t}$ and $\varepsilon_{\underline{\delta}}$ for some $\underline{\delta}\in\{0,1\}^r$.
\end{proof}

It is readily seen that $\varepsilon_{\underline{\delta}}$ is in non trivial degree if there exist $1\leq i \leq r$ such that $\delta_i=1$. Therefore tensoring by $\varepsilon_{\underline{\delta}}\not\simeq \mathbf{1}$ has no fixed points on the set of simple objects. As in \cref{sec:symmetric_center}, we want to (super)modularize the category $\mathcal{E}_{\underline{n},\xi^{-1}}$ and therefore we need that $\varepsilon_{\underline{\delta}}$ has a twist equal to $1$ for the chosen pivotal structure and evert $\underline{\delta}\in\{0,1\}^r$. We thus equip $\mathcal{D}_{n_i,\xi^{-1}}$ with a pivotal structure of the form $a_{d+2p_i,-}$ for some $p_i\in \mathbb{Z}$. The category $\mathcal{E}_{\underline{n},\xi^{-1}}$ is then equipped with a pivotal structure that we will denote by $a_{d+2\underline{p},-}$; the corresponding twist will be denoted by $\theta_{d+2\underline{p},-}$.

\begin{corollary}
  The symmetric center of $\mathcal{E}_{\underline{n},\xi^{-1}}$ equipped with the pivotal structure $a_{d+2\underline{p},-}$ is equivalent to $\Rep((\mathbb{Z}/2\mathbb{Z})^r,\underline{z})$ with $z_i = 1$ if $n_i\equiv d [2]$ and $z_i=0$ if $n_i\not\equiv d [2]$.

  The (super)modularization $\tilde{\mathcal{E}}_{\underline{n},\xi^{-1}}$  of $\mathcal{E}_{\underline{n},\xi^{-1}}$ has its objects parametrized by the set
  \[
    \tilde{E}_{\underline{n},d}=\left\{\underline{\lambda} \in \tilde{C}_{n_1,d}\times \cdots \times \tilde{C}_{n_r,d}\ \middle\vert\ \sum_{i=1}^r\langle\lambda_i,\varpi_{n_i}\rangle \equiv 0 [d]\right\}.
  \]
\end{corollary}

Note that the resulting category $\tilde{\mathcal{E}}_{\underline{n},\xi^{-1}}$ is a superfusion category as soon there exists $i$ such that $n_i$ and $d$ have the same parity. We summarize the results on the category $\tilde{\mathcal{E}}_{\underline{n},\xi^{-1}}$ and its modular invariants.

\begin{proposition}
  \label{prop:modular_inv_d1n}
  Recall that we endow the category the category $\tilde{\mathcal{E}}_{\underline{n},\xi^{-1}}$ with the pivotal structure $a_{d+2\underline{p},-}$. Then there exists a fourth root of unity $\omega$ such that the renormalized $S$-matrix of $\tilde{\mathcal{E}}_{\underline{n},\xi^{-1}}$ is given by
  \[
    \mathbb{S}_{\underline{\lambda},\underline{\mu}} = \frac{\omega}{\sqrt{d}}\prod_{i=1}^r\xi^{-\langle\lambda_i+\mu_i,(2p_i+d)\varpi_{n_i}\rangle-2p_i^2n_i}\frac{\sum_{w\in W_{n_i}}(-1)^{l(w)}\xi^{-2\langle w(\lambda_i+\rho_{n_i}),\mu_i+\rho_{n_i}\rangle}}{\sqrt{d}^{n_i}}
  \]
  for any $\underline{\lambda},\underline{\mu}\in \tilde{E}_{\underline{n},d}$. The twist on the simple object $X(\underline{\lambda})$ is given by $\xi^{-\sum_{i=1}^r\langle\lambda_i,\lambda_i+2\rho+(2p_i+d)\varpi_{n_i}\rangle}$.
\end{proposition}

\begin{proof}
  This follows immediately from \cref{thm:modular_data_gln}. The extra $\sqrt{d}$ at the denominator comes from the fact we work with the modularisation of the subcategory $\mathcal{E}_{\underline{n},\xi^{-1}}$ and not with the modularization of the whole category $\mathcal{D}_{\underline{n},\xi^{-1}}$.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../cat_exterior_powers_gd1n"
%%% End:

